NICP: Neural ICP for 3D Human Registration at Scale

Aligning a template to 3D human point clouds is a long-standing problem crucial for tasks like animation, reconstruction, and enabling supervised learning pipelines. Recent data-driven methods leverage predicted surface correspondences. However, they are not robust to varied poses, identities, or noise. In contrast, industrial solutions often rely on expensive manual annotations or multi-view capturing systems. Recently, neural fields have shown promising results. Still, their purely data-driven and extrinsic nature does not incorporate any guidance toward the target surface, often resulting in a trivial misalignment of the template registration. Currently, no method can be considered the standard for 3D Human registration, limiting the scalability of downstream applications. In this work, we propose a neural scalable registration method, NSR, a pipeline that, for the first time, generalizes and scales across thousands of shapes and more than ten different data sources. Our essential contribution is NICP, an ICP-style self-supervised task tailored to neural fields. NSR takes a few seconds, is self-supervised, and works out of the box on pre-trained neural fields. NSR combines NICP with a localized neural field trained on a large MoCap dataset, achieving the state of the art over public benchmarks. The release of our code and checkpoints provides a powerful tool useful for many downstream tasks like dataset alignments, cleaning, or asset animation.

==> sections/challenges_tables.tex <==


% \begin{wraptable}[8]{r}{0.6\linewidth}
% \scriptsize
%     \begin{center}	    	
% \begin{tabular}{lcc}
% 	          & FAUST$_{R}$ & FAUST$_{S}$          \\
% 		\hline
%   Uni-60 (\cite{marin2020correspondence})    &  3.52 &2.66   \\
%   Uni-2070 (\cite{marin2020correspondence}) 
%   &  3.49 & 2.62 \\
%   LVD    (\cite{corona2022learned})             & 4.78 & 3.54 \\
%   LVD+Chamfer \cite{corona2022learned} & 2.15 & 1.93 \\
%   \textbf{INLoVD (Ours)}    & \textbf{1.76} & \textbf{1.85} \\
% 	\end{tabular}
%     \end{center}
% 		\caption{\label{tab:comparison}
% 	Comparison with complete methods for human registration. They all use the same data and feature extractors.}
% \end{wraptable}

% \begin{wraptable}[6]{r}{0.5\linewidth}
% \scriptsize
% \vspace{-1cm}
%     \begin{center}    	
% 	\begin{tabular}{@{}lcc@{}}
% 		    & FAUST$_{R}$ & FAUST$_{S}$                    \\
%                 \hline
%                   OneShot        & 4.45          & 3.34         \\
%                   OneShot + INT  \textbf{(Ours)}     & \textit{3.64}            & \textit{3.15} \\
                  
%                 \hline
%                 LVD            & 4.78          & 3.54                \\ 
%                 LVD + INT     \textbf{(Ours)}    & \textit{3.40}            & \textit{2.81}  \\          \hline
%                 LoVD \textbf{(Ours)}    & \textbf{4.35} & \textbf{3.11} \\
%                 LoVD + INT    \textbf{(Ours)}    & \textit{\textbf{2.97}}   & \textit{\textbf{2.55}}   \\                  
%                 \hline
%           \end{tabular}
%            \end{center}
% 		\caption{\label{tab:backbones}
% 	NF comparisons. We show that our LoVD is the best NF out of the box, and our INT procedure improves all the backbones.}
% \end{wraptable}





% \begin{table}
% \begin{tabular}{c|c}

% \centering
% \scriptsize
% 	\begin{tabular}{@{}lrr@{}}
% 		          & INTRA & INTER          \\
% 		\hline
		
%         Loopreg (\cite{bhatnagar2020loopreg})    & 1.35     & 2.66 \\
%         Elementary (\cite{deprelle2019learning})  & 1.74     & 2.58 \\
%         UD2E-Net (\cite{Chen_2021_ICCV})          & 1.51     & 3.09 \\
%         \hline 
%         \textbf{INLoVD (Ours)}   & \textbf{1.06} & \textbf{2.26}\\
%         \hline
%         \hline 
%         DVM (multi-view)$^\dagger$  (\cite{kim2021deep})    &  1.19    & 2.37 \\
%         \hline
%         $^\dagger$: {Uses FAUST training set}
        
% 	\end{tabular}
%  	\captionof{table}{\label{fig:faust} Results from the public leaderboard on INTRA- and INTER-subject FAUST challenges.}

% & 

% \centering
% \scriptsize
% 	\begin{tabular}{@{}lr@{}}
% 		          & SHREC19          \\
% 		\hline
%         LIE (\cite{marin2020correspondence})   & 15.1   \\
%         GeoFMAP     (\cite{donati2020deep}) & 11.2\\
%         CorrNet3D (\cite{zeng2020corrnet3d})   & 9.6   \\
%         3DCoded    (\cite{groueix20183d}) & 10.3\\
%         Transmatch  (\cite{trappolini2021shape})& 6.1 \\
%         ReduceBasis (\cite{sundararaman2022reduced})& 4.8 \\ 
%         \hline 
%         \textbf{INLoVD \textbf{(Ours)}}         & \textbf{2.27}
% 	\end{tabular}
% 	\caption{\label{fig:shrec19} Results on SHREC19 challenge \cite{melzi2019shrec}. We improve the state of the art by 53\%}
%  \vspace{-0.1cm}
%  \end{tabular}
% \end{table}
